From Preferences to Principles: Rubric-Based Alignment for Grounded Knowledge Answers

Designing effective reward signals for open-domain question answering is challenging because high-quality responses must simultaneously satisfy multiple aspects of answer quality that are difficult to capture with a holistic scalar objective. We introduce a rubric-based reward framework that generates query-specific rubrics grounded in retrieved evidence and decomposed into multiple quality dimensions, providing fine-grained supervision during post-training. Averaged across three evaluation axes (composition, grounding, and instruction-following), our approach improves over the instruction-tuned baseline by 6.5% and over flat rubric variants by 4%, with consistent gains across all evaluation datasets. Conditioning rubrics on retrieved evidence improves factual support, while decomposing rubrics into quality-specific dimensions further improves coherence, organization, and adherence to query requirements. Our results show that grounded, multi-dimensional rubrics provide more effective reward supervision for complex open-domain question answering.

==> latex/diagram.tex <==
\begin{figure}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}[
  font=\sffamily,
  box/.style={
    rounded corners=4pt,
    draw=black,
    thick,
    fill=white,
    minimum height=1.15cm,
    align=center,
    font=\sffamily\footnotesize,
    inner sep=4pt
  },
  llmbox/.style={
    rounded corners=4pt,
    draw=#1,
    thick,
    fill=#1!10,
    minimum height=1.15cm,
    align=center,
    font=\sffamily\footnotesize,
    inner sep=4pt
  },
  s2box/.style={
    rounded corners=4pt,
    draw=black,
    thick,
    fill=white,
    minimum width=2.45cm,
    minimum height=1.65cm,
    text width=2.05cm,
    align=center,
    font=\sffamily\footnotesize,
    inner sep=2pt
  },
  s2llmbox/.style={
    rounded corners=4pt,
    draw=green!50!black,
    thick,
    fill=green!50!black!10,
    minimum width=2.45cm,
    minimum height=1.65cm,
    text width=2.05cm,
    align=center,
    font=\sffamily\footnotesize,
    inner sep=2pt
  },
  arrow/.style={-{Latex[length=2mm]}, thick},
  title/.style={font=\sffamily\bfseries\small, anchor=west}
]

\def\stageW{11.6cm}
\def\stageH{2.75cm}

% ================= Stage 1 =================
\node[
  rounded corners=6pt,
  draw=blue,
  very thick,
  fill=blue!4,
  minimum width=\stageW,
  minimum height=\stageH
] (stage1) at (0,0) {};

\node[title, text=blue!60!black]
at ([xshift=-5.45cm,yshift=0.95cm]stage1.center)
{Stage 1: Rubric Generation (Offline)};

\node[box, text width=2.3cm] (s1in) at (-3.7,-0.25)
{Query +\\Passages +\\Reference Answer};

\node[llmbox=blue, text width=2.4cm] (s1llm) at (0,-0.25)
{{\bfseries\color{blue!80!black} Strong LLM\\Rubric Generator}\\[2pt]
{\scriptsize (\textit{Generation} prompt)}};

\node[box, text width=2.5cm] (s1out) at (3.7,-0.25)
{Multi-Dimensional\\Grounded Rubrics};

\draw[arrow] (s1in) -- (s1llm);
\draw[arrow] (s1llm) -- (s1out);

% ================= Stage 2 =================
\node[
  rounded corners=6pt,
  draw=green!50!black,
  very thick,
  fill=green!50!black!4,
  minimum width=\stageW,
  minimum height=3.25cm
] (stage2) at (0,-3.45) {};

\node[title, text=green!40!black]
at ([xshift=-5.45cm,yshift=1.18cm]stage2.center)
{Stage 2: RL with Rubric-based Rewards};

\node[s2box] (policy) at (-4.15,-3.45)
{Policy\\Model};

\node[s2box] (rollout) at (-1.4,-3.45)
{Rollout\\Response};

\node[s2llmbox] (s2judge) at (1.4,-3.45)
{{\bfseries\color{green!60!black} LLM Judge}\\[2pt]
{\scriptsize (\textit{Judge} Prompt)}};

\node[s2box] (reward) at (4.15,-3.45)
{Combined\\Reward\\$R = R_{\text{rubric}}$\\$-\lambda L$};

\draw[arrow] (policy.east) -- (rollout.west);
\draw[arrow] (rollout.east) -- (s2judge.west);
\draw[arrow] (s2judge.east) -- (reward.west);

% RL loop
\draw[-{Latex[length=2mm]}, thick, green!50!black]
  (reward.south) -- (4.15,-4.65)
  -- node[midway, below, font=\sffamily\scriptsize\bfseries]
     {RL Policy Update}
  (-4.15,-4.65)
  -- (policy.south);

% Rubric criteria flow into RL judge
\draw[
  dashed,
  -{Latex[length=2mm]},
  thick,
  blue!70!black
]
(s1out.south) ..
controls +(0,-1.45) and +(0,1.1) ..
node[pos=0.72, right, yshift=-3pt, font=\sffamily\scriptsize\bfseries, text=blue!70!black]
{Rubrics}
(s2judge.north);

% Stage arrow
\draw[arrow] (stage1.south) -- (stage2.north);

% % ================= Optional Evaluation =================
% \node[
%   rounded corners=6pt,
%   draw=orange,
%   very thick,
%   dashed,
%   fill=orange!4,
%   minimum width=\stageW,
%   minimum height=2.55cm
% ] (optional) at (0,-6.75) {};

% \node[title, text=orange!70!black]
% at ([xshift=-5.45cm,yshift=0.82cm]optional.center)
% {Optional: Rubric Quality Evaluation (Offline)};

% \node[box, text width=2.0cm] (optin) at (-4.15,-6.95)
% {Candidate\\Responses\\+ Rubrics};

% \node[llmbox=orange, text width=1.9cm] (optjudge) at (-1.4,-6.95)
% {{\bfseries\color{orange!80!black} LLM Judge}\\[2pt]
% {\scriptsize (\textit{Judge} Prompt)}};

% \node[box, text width=1.9cm] (optscore) at (1.4,-6.95)
% {Rubric Score\\$\in [0,1]$};

% \node[box, dashed, text width=2.0cm] (optsbs) at (4.15,-6.95)
% {SBS\\Preference\\Labels};

% \node[
%   font=\sffamily\scriptsize\itshape,
%   text=orange!70!black,
%   anchor=south
% ] at ([yshift=2pt]optsbs.north)
% {Alignment Validation};

% \draw[arrow] (optin.east) -- (optjudge.west);
% \draw[arrow] (optjudge.east) -- (optscore.west);
% \draw[<->, thick] (optscore.east) -- (optsbs.west);

\end{tikzpicture}
}
\caption{Overview of the proposed rubric generation and training pipeline. See Appendix~\ref{app:prompts} for prompt templates, particularly Figure~\ref{fig:rubric-prompt} for \textit{Generation} prompt and Figure~\ref{fig:judge-prompt-1} for \textit{Judge} prompt.}
\label{fig:rubric_pipeline}
\end{figure}
